Dark Energy Survey Year 6 Results: Photometric Data Set for Cosmology

We describe the photometric data set assembled from the full six years of observations by the Dark Energy Survey (DES) in support of static-sky cosmology analyses. DES Y6 Gold is a curated data set derived from DES Data Release 2 (DR2) that incorporates improved measurement, photometric calibration, object classification and value added information. Y6 Gold comprises nearly $5000~{\rm deg}^2$ of $grizY$ imaging in the south Galactic cap and includes 669 million objects with a depth of $i_{AB} \sim 23.4$ mag at S/N $\sim 10$ for extended objects and a top-of-the-atmosphere photometric uniformity $< 2~{\rm mmag}$. Y6 Gold augments DES DR2 with simultaneous fits to multi-epoch photometry for more robust galaxy shapes, colors, and photometric redshift estimates. Y6 Gold features improved morphological star-galaxy classification with efficiency $98.6\%$ and contamination $0.8\%$ for galaxies with $17.5 < i_{AB} < 22.5$. Additionally, it includes per-object quality information, and accompanying maps of the footprint coverage, masked regions, imaging depth, survey conditions, and astrophysical foregrounds that are used for cosmology analyses. After quality selections, benchmark samples contain 448 million galaxies and 120 million stars. This paper will be complemented by online data access and documentation.

==> tables/extclass_performance.tex <==
\begin{deluxetable*}{l c c c c c c}
\tablewidth{0pt}
\tabletypesize{\tablesize}
\tablecaption{Performance of the morphological star/galaxy separation.
\label{tab:extclass_performance}}
\tablehead{
\colhead{Selection} & \hspace{1cm} & \multicolumn{2}{c}{$17.5 \leq \var{MAG\_AUTO\_I} \leq 22.5$} & \hspace{1cm} & \multicolumn{2}{c}{$16.5 \leq \var{MAG\_AUTO\_I} \leq 23.5$} \\
 & & \colhead{Efficiency} & \colhead{Contamination} & \hspace{1cm} & \colhead{Efficiency} & \colhead{Contamination}}
\startdata
& & \multicolumn{5}{c}{Galaxy Selection} \\
\hline
$2 \leq \var{EXT\_MASH} \leq 4$ & & 99.6\% & 1.3\% & & 99.2\% & 1.8\% \\
$3 \leq \var{EXT\_MASH} \leq 4$ & & 99.6\% & 1.3\% & & 98.8\% & 1.6\% \\
$\var{EXT\_MASH} = 4$           & & 98.6\% & 0.8\% & & 96.3\% & 1.0\% \\
\hline
$2 \leq \var{EXT\_XGB} \leq 4$  & & 99.0\% & 0.5\% & & 97.7\% & 1.0\% \\
$3 \leq \var{EXT\_XGB} \leq 4$  & & 98.3\% & 0.4\% & & 96.2\% & 0.8\% \\
$\var{EXT\_XGB} = 4$            & & 96.7\% & 0.3\% & & 92.5\% & 0.5\% \\
\hline
$\var{XGB\_PRED} \leq 0.65$        & & 99.6\% & 1.1\% & & 99.5\% & 2.1\% \\
$\var{XGB\_PRED} \leq 0.50$        & & 99.6\% & 0.9\% & & 99.3\% & 1.7\% \\
$\var{XGB\_PRED} \leq 0.058$       & & 98.6\% & 0.4\% & & 96.7\% & 0.8\% \\
\hline
& & \multicolumn{5}{c}{Stellar Selection} \\
\hline
$0 = \var{EXT\_MASH}$           & & 89.2\% & 0.7\% & & 80.0\% & 2.0\% \\
$0 \leq \var{EXT\_MASH} \leq 1$ & & 94.6\% & 1.5\% & & 88.9\% & 5.2\% \\
$0 \leq \var{EXT\_MASH} \leq 2$ & & 94.7\% & 1.6\% & & 90.2\% & 7.1\% \\
\hline
$0 = \var{EXT\_XGB}$            & & 92.1\% & 1.0\% & & 79.3\% & 1.5\% \\
$0 \leq \var{EXT\_XGB} \leq 1$  & & 98.0\% & 4.0\% & & 94.3\% & 12.5\% \\
$0 \leq \var{EXT\_XGB} \leq 2$  & & 98.5\% & 6.4\% & & 95.6\% & 19.2\% \\
\hline
$\var{XGB\_PRED} > 0.906$       & & 89.2\% & 0.9\% & & 74.8\% & 1.1\% \\
$\var{XGB\_PRED} > 0.76$        & & 94.6\% & 1.2\% & & 84.2\% & 2.2\% \\
$\var{XGB\_PRED} > 0.75$        & & 94.7\% & 1.3\% & & 84.6\% & 2.2\% \\
\hline
\enddata
\tablecomments{The \var{EXT\_XGB} classes were assigned to give a similar number of objects per class as \var{EXT\_MASH}. The \var{XGB\_PRED} cuts were tuned to give the same completeness as \var{EXT\_MASH} on the specific evaluation data set used.}
\end{deluxetable*}

